Simulating strongly interacting Hubbard chains with the Variational Hamiltonian Ansatz on a quantum computer

Hybrid quantum-classical algorithms have been proposed to circumvent noise limitations in quantum computers. Such algorithms delegate only a calculation of the expectation value to the quantum computer. Among them, the Variational Quantum Eigensolver (VQE) has been implemented to study molecules and condensed matter systems on small size quantum computers. Condensed matter systems described by the Hubbard model exhibit a rich phase diagram alongside exotic states of matter. In this manuscript, we try to answer the question: how much of the underlying physics of a 1D Hubbard chain is described by a problem-inspired Variational Hamiltonian Ansatz (VHA) in a broad range of parameter values ? We start by probing how much does the solution increases fidelity with increasing ansatz complexity. Our findings suggest that even low fidelity solutions capture energy and number of doubly occupied sites well, while spin-spin correlations are not well captured even when the solution is of high fidelity. Our powerful simulation platform allows us to incorporate a realistic noise model and shows a successful implementation of noise-mitigation strategies - post-selection and the Richardson extrapolation. Finally, we compare our results with an experimental realization of the algorithm on IBM Quantum's ibmq_quito device.

==> tikzlibraryquantikz.code.tex <==
%This is the quantikz library for typesetting quantum circuits using LaTeX/Tikz. version 0.9.6
% Written by Alastair Kay, 2018. Published under a CC-BY-4.0 licence
% Please email me (alastair.kay@rhul.ac.uk) with any bug reports or feature requests.
% If you find this library useful, please cite its usage in your work, using arXiv:1809.03842, and possibly the DOI: 10.17637/rh.7000520.
% Usage is at your own risk.

%version 0.9.6:
%	changed packaging so there isn't a compile warning any more
%	modified the meter command so that \meter[draw=blue]{} colours everything blue, not just outline.
%	added trash command
%	added \ctrlbundle command so that \ctrl works well with \qwbundle[alternate]. If you supple \ctrlbundle[2]{}, then the bundle only contains 2 wires instead of the default of 3
%	\qwbundle[alternate] now also works with the parameter \qwbundle[alternate=2] to only have 2 wires in the bundle.
%	added \midstick. Works a bit like rstick and lstick, but reserves space for the text. Can choose to have brackets=none|left|right|both (default is both). Gives better method for circuit identities and other things.
%	added "align equals at" key for setting circuit identities (specifies wire number that should line up with equals. can be non-integer)
%	added makeebit command. accepts one parameter which is the text. Haven't got tyling and different angles of the split working yet.
%   added bundle option to supplement nwires and cwires.
%	fixed bug where you couldn't put a wire command after the declaration of a multi-qubit gate command.
%version 0.9.5:
%	fixed bug which meant multi-wire gates didn't work outside of an environment such as center.
%version 0.9.4:
%	added nwires and cwires options to gate command to simulate qcircuit's nphantom and cphantom
%	vertical text options for slice labels.
%	replaced macro for measuring width and height for greater reliability. disable auto spacing now unnecessary as things like \sqrt{} work in the gate label.
%	investigated possibility of high labels (multi-line labels, particularly for a multi-qubit gate). key disable auto height introduced.
%	now provides a quantikz environment, which is theoretically compatible with tikz' external library (entirely untested). Can still use tikzcd environment otherwise.
%	removed a tikzcd customisation fixing the baseline for one row circuits as this was messing with any manual attempts to adjust the baseline.
%version 0.9.3:
%	adjusted spacing of gate operation between in-circuit and overlay so that transparency looks better
%	Other gate spacing adjustments. multi-qubit gates in particular should look better. 'disable auto spacing' can switch this off, particularly for use with things like \sqrt{} in the multi-qubit gate label, which will throw a weird error.
%	gate command now takes two further optional parameters: minimum width and minimum height for each cell.
%	some consolidation of styling commands
%	global keys 'transparent' and 'thin lines' added. 'thin lines' gives a look more similar to the original QCircuit.
%version 0.9.2:
%	made 'wires' the default key, so [wires=2] now becomes [2]
%	added 'slice title', 'slices style', 'slices label style' key to control titles of slices under 'slice all'
%	better access to positioning of gategroup label.
%	now arXiv compatible (that was a challenge! they use old versions of packages)
%Previous versions:
%version 0.9.1:
%	added \cwbend gate for cornering classical wires.
%	made size of strike through for multiqubit gates stylable via the keys /quantikz/Strike Height/ and /quantikz/Strike Width/
%	added new \gate[swap] variant of swap (nearest-neighbour only).
%version 0.9.0:
%original release.

%\ProvidesPackage{quantikz}[2020/04/27 typeset quantum circuit diagrams]

% Package(s) to include
\RequirePackage{xargs,ifthen,xstring,xparse,etoolbox,mathtools,pgfmath}
\RequirePackage{environ} %in an attempt to help with compatibility with the external library of tikz.
%\RequirePackage{tikz}
\usetikzlibrary{cd,decorations.pathreplacing,calc,positioning,fit,shapes.symbols,decorations.pathmorphing,shapes.misc,backgrounds,decorations.markings,math}

\newlength{\myl}
\newlength{\myh}
\newlength{\myd}

%\makeatletter
\newcounter{aaa}
\tikzset{
  apply/.style args={#1 except on segments #2}{postaction={
      /utils/exec={
        \@for\mattempa:=#2\do{\csdef{aaa@\mattempa}{}}
        \setcounter{aaa}{0}
      },
      decorate,decoration={show path construction,
        moveto code={},
        lineto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path[#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
        curveto code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) .. controls
            (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
            ..(\tikzinputsegmentlast);
          }
        },
        closepath code={
          \stepcounter{aaa}
          \ifcsdef{aaa@\theaaa}{}{
            \path [#1] (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
          }
        },
      },
    },
  },
}
%test if item is in list of item. Probably better ways to do this, but I could get this version to work.
\newcommand*{\IfInList}[2]{%
	\gdef\memory{0}
	\edef\arg{#1}
	 \foreach \q in #2 {%
	 	\ifthenelse{\q=\arg}{%
	 		\gdef\memory{1}
	 	}{}
	 }
	\ifthenelse{\memory=1} {%
		\expandafter\@firstoftwo
	}{%
		\expandafter\@secondoftwo
	}
}
%define the quantikz environment. I need this to facilitate the external library
\NewEnviron{quantikz}[1][]{%
  \def\@temp{\tikzcd@[#1]\BODY}%
  \expandafter\@temp\endtikzcd
}
\def\temp{&} \catcode`&=\active \let&=\temp
%
%commands for putting in text vertically
\protected\def\vvv#1{\leavevmode\bgroup\vbox\bgroup\xvvv#1\relax}
%
\def\xvvv{\afterassignment\xxvvv\let\tmp= }
%
\def\xxvvv{%
% \ifx\tmp\@sptoken\egroup\ \vbox\bgroup\let\next\xvvv
% \else
\ifx\tmp\relax\egroup\egroup\let\next\relax
 \else
\hbox to 1.1em{\hfill\tmp\hfill}% centred
\let\next\xvvv\fi%\fi
\next}
%end of commands for putting text vertically
%
\long\def\ifnodedefined#1#2#3{%
    \@ifundefined{pgf@sh@ns@#1}{#3}{#2}%
}
%I don't think this is used any more
% \newcommand\getwidth[1]{
% 	\pgfkeys{minimum width=0pt}%
% 	\pgfkeys{/quantikz,#1}
% 	\pgfkeysgetvalue{/quantikz/minimum width}{\minwidth}
% 	\minwidth
% }

%find the vertical position of the middle of an equals sign
%https://tex.stackexchange.com/questions/355680/how-can-i-vertically-align-an-equals-sign-in-a-tikz-node/355686
\pgfmathsetmacro\MathAxis{height("$\vcenter{}$")}

%the main gate command
\DeclareExpandableDocumentCommand{\gate}{O{}O{1.5pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner sep=4pt,minimum width=#2,minimum height=#3]|%
 	\edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
 	%reset macros that are going to be set by the options
 	\edef\options{row=\n,col=\m,#1}
 	\def\toswap{0}%
 	\def\DisableMinSize{0}%
 	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
 	%import options passed as parameters
  	\pgfkeys{/quantikz,#1}%
 	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
 	\pgfkeysgetvalue{/quantikz/style}{\a}
 	\pgfkeysgetvalue{/quantikz/label style}{\b}
 	\pgfkeysgetvalue{/quantikz/cwires}{\mylist}
 	\pgfkeysgetvalue{/quantikz/nwires}{\nowires}
 	\pgfkeysgetvalue{/quantikz/bundle}{\bundle}
 	\ifthenelse{\toswap=1}{%if it's a swap gate...
 		\def\quantwires{2}
 		\phantom{wide}
 		\settowidth{\myl}{$wide$}
 		\settoheight{\myh}{$wide$}
 		\settodepth{\myd}{$wide$}
 	}{%not a swap gate
 		\settowidth{\myl}{$#4$}
 		\ifthenelse{\DisableMinSize=1}{%disable automatic size detection. Use $U$ instead.
 			\phantom{U}
 			\settoheight{\myh}{$U$}
 			\settodepth{\myd}{$U$}
 		}{%automatically get width and height of label
 			\phantom{#4}
 			\settoheight{\myh}{$#4$}
 			\settodepth{\myd}{$#4$}
 		}
 	}
%	
 	\IfInList{1}{\mylist}{\cw}{\IfInList{1}{\nowires}{}{\IfInList{1}{\bundle}{\qwbundle[alternate]{}}{\qw}}}%do we need classical, no wire, or quantum wire?
 	\edef\k{\the\numexpr\n+\quantwires-1\relax}
 	\edef\mn{\the\numexpr\m-1\relax}
 	\ifthenelse{\quantwires=1}{}{%more than 1 wire on gate. iterate through each wire
 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	    \edef\newcom{\noexpand\vcwhexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomb{\noexpand\vqwexplicit{\i-\m}{\i-\mn}}
       	\edef\newcomc{\noexpand\vqbundleexplicit{\i-\m}{\i-\mn}}
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		\IfInList{\val}{\mylist}{\newcom}{\IfInList{\val}{\nowires}{}{\IfInList{\val}{\bundle}{\newcomc}{\newcomb}}}%do we need classical, no wire, or quantum wire?
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={max(\the\myl+8pt,#2)}}}}%
 		\dotikzset%
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}%
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}%
 	}
 			%apply auto height to last row only. unsetting already handled above.
 		   \globaldefs=1%
 		   \edef\dotikzset{\noexpand\tikzset{row \k\space column \m/.append style={minimum height={max(\the\myh+\the\myd+8pt,#3)}}}}%
 		   \dotikzset%
 		   \globaldefs=0%
%		
 	}
 	%call deferred gate command. to be executed after the tikzcd matrix stuff is completed
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gate@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\a\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\b\expandafter}\expandafter{\options}{#4}
	}
}

%deferred gate command. draws a box around all included cells. this is not part of the matrix, but comes afterwards.
\newcommand{\gate@end}[4]{
	\pgfkeys{/quantikz,wires=1}
	\def\toswap{0}
	\def\DisableMinSize{0}
 	\pgfkeys{/quantikz,#3}%import options
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\ifthenelse{\toswap=1}{\def\quantwires{2}}{}
	\xdef\LoopGG{}
	%create a list of cell names to be included in this grouped gate
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGG{\LoopGG(\tikzcdmatrixname-\n-\col)}
		}{}
	}
	\ifthenelse{\toswap=1}{
		\node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,#1] {\hphantom{Wide}};
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\row-\col.center) to[out=0,in=180] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [line width=3pt,white,shorten >=0.9pt,shorten <=0.9pt] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
		\draw [thickness] (group\tikzcdmatrixname-\row-\col.east|-\tikzcdmatrixname-\row-\col.center) to[out=180,in=0] (group\tikzcdmatrixname-\row-\col.west|-\tikzcdmatrixname-\the\numexpr\row+1\relax-\col.center);
	}{
	%the actual gate drawing command
	  \node (group\tikzcdmatrixname-\row-\col) [fit=\LoopGG,operator,inner sep=0pt,label={[gg label,#2]$#4$},#1] {\hphantom{$#4$}};
	}
}

%ghost will get height correct if can't be automatically assigned.
\DeclareExpandableDocumentCommand{\ghost}{O{}O{0pt}O{1.5pt}m}{%optional parameter contains styling info. compulsory is gate text.
	|[inner ysep=4pt,minimum width=#2,minimum height=#3]| \vphantom{#4}
}


%single slice
\newcommand\slice[2][]{%
	%\edef\currcol{\the\pgfmatrixcurrentcolumn}
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
 	\edef\options{\pgfkeysvalueof{/quantikz/style}}
 	\edef\opts{\pgfkeysvalueof{/quantikz/label style}}
	\edef\n{\the\pgfmatrixcurrentcolumn}
	%\expandafter\show\n
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendslices\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}}
%deferred slice command
\newcommand{\slice@end}[4]{
	\edef\top{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row1.north)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row1.north)$)}
	\edef\bottom{($1/2*(\tikzcdmatrixname-col#1.east |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+1/2*(\tikzcdmatrixname-col\the\numexpr#1+1\relax.west |- \tikzcdmatrixname-row\the\pgfmatrixcurrentrow.south)+(0,-3pt)$)}
	\expandafter\expandafter\expandafter\make@slice\expandafter\expandafter\expandafter{\expandafter\top\expandafter}\expandafter{\bottom}{#4}{#2}{#3}
}
\newcommand{\make@slice}[5]{
	\draw[slice,#4] #1 to node[pos=0,inner sep=4pt,anchor=south,color=black,#5] {#3} #2;
}
%deferred command which will slice everything
\newcommand{\sliceallr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\pgfkeysvalueof{/tikz/slice titles}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}
%deferred slice command with vertical text
\newcommand{\sliceallvr}{
	\edef\sstyle{\pgfkeysvalueof{/tikz/slice style}}
	\edef\slstyle{\pgfkeysvalueof{/tikz/slice label style}}
	\foreach \n in  {2,...,\the\numexpr\pgfmatrixcurrentcolumn-1-\pgfkeysvalueof{/tikz/remove end slices}\relax} {
		\edef\col{\the\numexpr\n-1\relax}
		\edef\title{\vvv{\pgfkeysvalueof{/tikz/slice titles}}}
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\slice@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\n\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\sstyle\expandafter}\expandafter{\slstyle}{\title}
	}
}

%labelling of inputs
\newcommand\lstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupinput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%labelling of outputs
\newcommand\rstick[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}

\newcommand\midstick[2][]{%
	\hphantom{\text{gg#2gg}}\ %leave enough space for whatever text we've inserted
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/label style}{\options}
	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	 \edef\n{\the\pgfmatrixcurrentrow} %the row
 	\edef\m{\the\pgfmatrixcurrentcolumn} %the column
	\edef\mn{\the\numexpr\m-1\relax}
	\edef\k{\the\numexpr\n+\quantwires-1\relax}
	\settowidth{\myl}{gg#2gg}
	%if more than 1 wire, need to reserve space for each wire
	\ifthenelse{\quantwires=1}{}{
	 	\foreach \i in {\the\numexpr\n+1\relax,...,\k} {
 	 	\edef\val{\the\numexpr\i+1-\n\relax}
 		%apply auto width to the cell, and make sure we unset the setting so that it doesn't apply to later circuits.
 		%I think use of globaldefs in this way is very slow, but I don't know of a better way.
 		\globaldefs=1
 		\edef\dotikzset{\noexpand\tikzset{row \i\space column \m/.append style={minimum width={\the\myl}}}}
 		\dotikzset
 		\edef\undotikzset{\noexpand\tikzset{row \i\space column \m/.style={}}}
      	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendglobals\expandafter{\undotikzset}
      	\globaldefs=0
 	}
%		
 	}
	%\edef\n{\the\pgfmatrixcurrentrow}
	%\edef\m{\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendsavedpaths\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\groupoutput@mid\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred labelling of inputs
\newcommand{\groupinput@end}[4]{%basic data as keys, lable options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGI{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
	\ifnodedefined{\tikzcdmatrixname-\n-\col}{
		\xdef\LoopGI{\LoopGI(\tikzcdmatrixname-\n-\col)} 
		}{}
		}
	\ifthenelse{\quantwires=1} {
		\node (ingr-\row) [fit=\LoopGI, inner sep=0pt,label={[align=center,#2]left:#4}] {};
	}{
	\node (ingr-\row) [fit=\LoopGI, inner sep=0pt] {};
	\draw[dm,#3] ($(ingr-\row.north west)+(-0.1cm,0.1cm)$) to node[midway,align=center,anchor=east,xshift=-0.1cm,#2] {#4} ($(ingr-\row.south west)+(-0.1cm,-0.1cm)$);
	}
} %
%deferred labelling of outputs
\newcommand{\groupoutput@end}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (outgr-\row) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]right:#4}] {};
	}{
	\node (outgr-\row) [fit=\LoopGO, inner sep=0pt] {};
	\draw[dd,#3] ($(outgr-\row.north east)+(0.1cm,0.1cm)$) to node[midway,align=center,anchor=west,xshift=0.1cm,#2] {#4} ($(outgr-\row.south east)+(0.1cm,-0.1cm)$);
	}
} %
%deferred labelling in the middle of circuits
\newcommand{\groupoutput@mid}[4]{%basic data as keys, label options, brace options, text
	\pgfkeys{/quantikz,wires=1}
	\def\leftbrace{1}\def\rightbrace{1}
 	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
	\xdef\LoopGO{}
	\foreach \n in  {\row,...,\the\numexpr\row+\quantwires-1\relax} {
		\ifnodedefined{\tikzcdmatrixname-\n-\col}{
			\xdef\LoopGO{\LoopGO(\tikzcdmatrixname-\n-\col)} 
		}}
		\ifthenelse{\quantwires=1} {
		\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[align=center,#2]#4}] {};
	}{
	\node (midgr-\row-\col) [fit=\LoopGO, inner sep=0pt,label={[anchor=mid,#2]center:#4}] {};
	\ifthenelse{\rightbrace=1}{
	\draw[dm,#3] ($(midgr-\row-\col.north east)+(-0.1cm,0.05cm)$) to ($(midgr-\row-\col.south east)+(-0.1cm,-0.05cm)$);
	}{}
	\ifthenelse{\leftbrace=1}{
	\draw[dd,#3] ($(midgr-\row-\col.north west)+(0.1cm,0.05cm)$) to ($(midgr-\row-\col.south west)+(0.1cm,-0.05cm)$);
	}{}
	}
} %
%inputs and outputs within a multi-wire gate
\newcommand\gateinput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}%
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}%
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mginput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
\newcommand\gateoutput[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/label style}{\options}
 	\pgfkeysgetvalue{/quantikz/braces}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\mgoutput@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred functions for the above
\newcommand{\mginput@end}[4]{%collected options,label style, brace style,text
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0,0cm)$)[leftinternal,#2]{#4};
}{%
%\show\quantwires
\draw[dd,#3] ($(\cell.west |- \tikzcdmatrixname-\row-\col.west)+(0.1cm,0.1cm)$) to node[leftinternal,midway,#2] {#4} ($(\cell.west |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.west)+(0.1cm,-0.1cm)$);
}
} %
\newcommand{\mgoutput@end}[4]{%
	\pgfkeys{/quantikz,wires=1}
 	\pgfkeys{/quantikz,#1}%
 	\edef\quantwires{\pgfkeysvalueof{/quantikz/wires}}
	%\pgfkeysgetvalue{/quantikz/wires}{\quantwires}
	\pgfkeysgetvalue{/quantikz/row}{\row}
	\pgfkeysgetvalue{/quantikz/col}{\col}
%can we find the gategroup node?
\xdef\cell{group\tikzcdmatrixname-1-\col}
\foreach \n in {\row,...,1} {%
	%test if node group-\n-#2 exists
	\ifnodedefined{group\tikzcdmatrixname-\n-\col}{%
    	\xdef\cell{group\tikzcdmatrixname-\n-\col}
    	\breakforeach
	}{}
}
\ifthenelse{\quantwires=1}{%
	\node at ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(0,0cm)$)[rightinternal,#2]{#4};
}{%
\draw[dm,#3] ($(\cell.east |- \tikzcdmatrixname-\row-\col.east)+(-0.1cm,0.1cm)$) to node[rightinternal,midway,#2] {#4} ($(\cell.east |- \tikzcdmatrixname-\the\numexpr\row+\quantwires-1\relax-\col.east)+(-0.1cm,-0.1cm)$);
}
} %

%wave command
\newcommand\wave[1][]{%
	\edef\n{\the\pgfmatrixcurrentrow}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendslices\expandafter{%
		\expandafter\wave@end\expandafter{\n}{#1}%
	}
}
%deferred wave
\newcommand{\wave@end}[2]{
	\node (wave-#1) [fit=(\tikzcdmatrixname-row#1),wave,#2] {};
}

\DeclareDocumentCommand{\makeebit}{O{-45}O{}m}{
	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!{0.5/cos(#1)}!#1:(\tikztotarget)$) node [anchor=east,style={#2}]{#3} -- (\tikztotarget) }]{d}
}

% \newcommand{\makeebit}[2][-45]{
% 	\arrow[arrows,line cap=round,to path={(\tikztostart) -- ($(\tikztostart)!0.707!#1:(\tikztotarget)$) node [anchor=east]{#2} -- (\tikztotarget) }]{d}
% }

%put a border around a group of gates
\newcommand\gategroup[2][]{%
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=}
	\pgfkeys{/quantikz,#1}%
	\edef\newoptions{row=\the\pgfmatrixcurrentrow,col=\the\pgfmatrixcurrentcolumn,#1}
 	\pgfkeysgetvalue{/quantikz/style}{\options}
 	\pgfkeysgetvalue{/quantikz/label style}{\opts}
	\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\pgfutil@g@addto@macro\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\tikzcd@atendlabels\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
		\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\gategroup@end\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{\expandafter\expandafter\expandafter\newoptions\expandafter\expandafter\expandafter}\expandafter\expandafter\expandafter{\expandafter\options\expandafter}\expandafter{\opts}{#2}%
	}
}
%deferred gate group command
\newcommand{\gategroup@end}[4]{%options, gate style, text style, text
	\pgfkeys{/quantikz,wires=1,style=,label style=,braces=,steps=1}%
	\edef\background{0}%
	\pgfkeys{/quantikz,#1}%
	\pgfkeysgetvalue{/quantikz/wires}{\quantwires}%
	\pgfkeysgetvalue{/quantikz/row}{\row}%
	\pgfkeysgetvalue{/quantikz/col}{\col}%
	\pgfkeysgetvalue{/quantikz/steps}{\steps}%
	\edef\fit{(\tikzcdmatrixname-col\col.west |- \tikzcdmatrixname-row\row.north)(\tikzcdmatrixname-col\the\numexpr\col+\steps-1\relax.east |- \tikzcdmatrixname-row\the\numexpr\row+\quantwires-1\relax.south)}%
	\ifthenelse{\background=1}{%
		\begin{scope}[on background layer]\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};\end{scope}
	}{%
		\node (ggroup-\row-\col) [fit=\fit,ggroup,label={[group label,#3]:#4},#2] {};
	}
}

%use for fudging classical wires that have horizontal and vertical sections
\newcommand{\cwbend}[1]{
	\vcw{#1}\cw
	\edef\cell{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\expandafter\pgfutil@g@addto@macro\expandafter\tikzcd@atendlabels\expandafter{%
		\expandafter\latephase@end\expandafter{\cell}
	}
}

\newcommand{\latephase@end}[1]{
	\node [phase,inner sep=2pt] at (\tikzcdmatrixname-#1) {};
}

%patch tikzcd to allow for multiple layers of commands
\patchcmd\tikzcd@{\tikzpicture}{\def\toslice{0}\def\vert{0}
 \begin{tikzpicture}}{}{}
\patchcmd\tikzcd@
    {\global\let\tikzcd@savedpaths\pgfutil@empty}
    {\global\let\tikzcd@savedpaths\pgfutil@empty
    \global\let\tikzcd@atendsavedpaths\pgfutil@empty
    \global\let\tikzcd@atendlabels\pgfutil@empty
    \global\let\tikzcd@atendslices\pgfutil@empty
    \global\let\tikzcd@atendglobals\pgfutil@empty
    \pgfutil@g@addto@macro\tikzcd@savedpaths\DivideRowsCols
    %\pgfmathsetmacro{\mname}{random(100000)}
    \ifthenelse{\toslice=1}{\ifthenelse{\vert=0}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallr}{\pgfutil@g@addto@macro\tikzcd@atendslices\sliceallvr}}{}
    }{}{}

%this patching works on modern systems, but I believe is incompatible with the old version that arXiv is running
%\patchcmd\endtikzcd{\tikzcd@savedpaths}{\tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals}}{}{}

%instead, completely redefine the function
\def\endtikzcd{%
  \pgfmatrixendrow\egroup%
  \pgfextra{\global\let\tikzcdmatrixname\tikzlastnode};%
  \tikzcdset{\the\pgfmatrixcurrentrow-row diagram/.try}%
  \begingroup%
    \pgfkeys{% `quotes' library support
      /handlers/first char syntax/the character "/.initial=\tikzcd@forward@quotes,%
      /tikz/edge quotes mean={%
        edge node={node [execute at begin node=\iftikzcd@mathmode$\fi,%$
                         execute at end node=\iftikzcd@mathmode$\fi,%$
                         /tikz/commutative diagrams/.cd,every label,##2]{##1}}}}%
    \let\tikzcd@errmessage\errmessage% improve error messages
    \def\errmessage##1{\tikzcd@errmessage{##1^^J...^^Jl.\tikzcd@lineno\space%
        I think the culprit is a tikzcd arrow in cell \tikzcd@currentrow-\tikzcd@currentcolumn}}%
    \tikzcd@before@paths@hook%
    \tikzcd@savedpaths\tikzcd@atendsavedpaths\tikzcd@atendlabels\tikzcd@atendslices{\globaldefs=1\tikzcd@atendglobals\globaldefs=0}%I just added stuff here instead
  \endgroup%
  \end{tikzpicture}%
  \ifnum0=`{}\fi}


%end patching
%\makeatother

%this command runs after we've finished the matrix, and makes unified cells for each row and each column. This allows much nicer alignment of large boxes.
\newcommand{\DivideRowsCols}{
	\foreach \n in {1,...,\the\pgfmatrixcurrentrow} {%for each row, construct a master cell that contains all entries
	\xdef\LoopRow{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentcolumn}{
			\ifnodedefined{\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(\tikzcdmatrixname-\n-\m)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\n-\m}{
				\xdef\LoopRow{\LoopRow(group\tikzcdmatrixname-\n-\m)}
			}{}
	}
	\node (\tikzcdmatrixname-row\n) [fit=\LoopRow] {};
	}
	\foreach \n in {1,...,\the\pgfmatrixcurrentcolumn} {%for each column, construct a master cell that contains all entries
	\xdef\LoopCol{}
		\foreach \m in {1,...,\the\pgfmatrixcurrentrow}{
			\ifnodedefined{\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(\tikzcdmatrixname-\m-\n)}
			}{}
			\ifnodedefined{group\tikzcdmatrixname-\m-\n}{
				\xdef\LoopCol{\LoopCol(group\tikzcdmatrixname-\m-\n)}
			}{}
	}
	\node (\tikzcdmatrixname-col\n) [fit=\LoopCol] {};
	}
}

%take a parameter, row number, where we want to set the baseline. if not integer, use the two rows spanned
\providecommand{\setmiddle}[1]{%
\IfInteger{#1}{
\pgfmathtruncatemacro\wholepart{floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]\noexpand\tikzcdmatrixname-\wholepart-1.base)}
}}
%\show\temp
\temp
}{%
\pgfmathtruncatemacro\wholepart{floor(#1)}
\pgfmathtruncatemacro\neighbour{floor(#1)+1}
\pgfmathsetmacro\fractionalpart{#1-floor(#1)}
\edef\temp{\noexpand\tikzset{%
/tikz/baseline={([yshift=-\MathAxis]$(\noexpand\tikzcdmatrixname-\wholepart-1.base)!\fractionalpart!(\noexpand\tikzcdmatrixname-\neighbour-1.base)$)}
}}
%\show\temp
\temp
}
}

%initialise all the pgfkeys for key=value parameter passing in macro options

\pgfkeys{/tikz/slice all/.code={\def\toslice{1}},/tikz/remove end slices/.initial=0,/tikz/slice titles/.initial={\col},/tikz/slice style/.initial={},/tikz/slice label style/.initial={},/tikz/thin lines/.code={\resetstyles},/tikz/transparent/.code={\maketransparent},/tikz/vertical slice labels/.code={\def\vert{1}},/tikz/align equals at/.code={\setmiddle{#1}}}
\pgfkeys{/quantikz/.is family,/quantikz,%
.unknown/.style={%
	/quantikz/wires=\pgfkeyscurrentname
},%
wires/.initial=1,%
style/.initial={},label style/.initial={},braces/.initial={},background/.code={\def\background{1}},alternate/.default=1,alternate/.code={\def\helper{#1}},row/.initial=1,col/.initial=1,steps/.initial=1,Strike Width/.initial=0.08cm,Strike Height/.initial=0.12cm,swap/.code={\def\toswap{1}},disable auto height/.code={\def\DisableMinSize{1}},cwires/.initial={-1},nwires/.initial={-1},bundle/.initial={-1},brackets/.is choice,brackets/.initial=both}
\pgfkeys{/quantikz,brackets/.cd,none/.code={\def\leftbrace{0}\def\rightbrace{0}},left/.code={\def\leftbrace{1}\def\rightbrace{0}},right/.code={\def\leftbrace{0}\def\rightbrace{1}},both/.code={\def\leftbrace{1}\def\rightbrace{1}}}

%my standard Dirac notation commands. can be overridden by user.
\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right |}}
\providecommand{\proj}[1]{\ensuremath{\ket{#1}\!\bra{#1}}}
\providecommand{\braket}[2]{\ensuremath{\left\langle#1\middle|#2\right\rangle}}

%single qubit operations
\newcommand{\phantomgate}[1]{|[linecont,thickness, inner ysep=3pt]| \phantom{#1} \qw}
\newcommand{\hphantomgate}[1]{|[linecont,minimum size=1.5em,thickness]| \hphantom{#1} \qw}
\newcommand{\push}[1]{#1 \qw}
\newcommand{\alias}[1]{|[alias=#1]|}
\DeclareExpandableDocumentCommand{\phase}{O{}m}{|[phase,#1,label={[phase label,#1]#2}]| {} \qw}
\DeclareExpandableDocumentCommand{\control}{O{}m}{|[phase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\ocontrol}{O{}m}{|[ophase,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targ}{O{}m}{|[circlewc,#1]| {} \qw}
\DeclareExpandableDocumentCommand{\targX}{O{}m}{|[crossx2,#1]| {} \qw}
\newcommand{\linethrough}{|[linecont, inner ysep=3pt]| }

%measuring
\DeclareExpandableDocumentCommand{\meter}{O{}{m}}{|[meter,label={[my label]#2},#1]| {} \qw}
\DeclareExpandableDocumentCommand{\measuretab}{O{}{m}}{|[measuretab,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\meterD}{O{}{m}}{|[meterD,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\measure}{O{}{m}}{|[measure,#1]| {#2} \qw}
\DeclareExpandableDocumentCommand{\trash}{O{}{m}}{|[trash,label={below:#2},#1]| {} \qw}


%controlled gates
\def\ctrl#1{\control{}	\vqw{#1}}
\DeclareExpandableDocumentCommand{\ctrlbundle}{O{1}O{}m}{|[phase bundle,#2]| {} \vqw{#3}\qwbundle[alternate=#1]{}}
\def\octrl#1{\ocontrol{}\vqw{#1}}
\def\swap#1{%
	\targX{}
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicitcenter\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}

%vertical wires
%classical vertical wire, relative positioning
\newcommand{\vcw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vcwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%vertical quantum wire, relative positioning
\newcommand{\vqw}[1]{
	\edef\start{\the\pgfmatrixcurrentrow-\the\pgfmatrixcurrentcolumn}
	\edef\end{\the\numexpr#1+\pgfmatrixcurrentrow\relax-\the\pgfmatrixcurrentcolumn}
	\expandafter\expandafter\expandafter\vqwexplicit\expandafter\expandafter\expandafter{\expandafter\start\expandafter}\expandafter{\end}
}
%quantum wire, absolute positioning
\newcommand{\vqwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {}
}
\newcommand{\vqbundleexplicit}[2]{
	\arrow[from=#1,to=#2,arrows] {} \arrow[from=#1,to=#2,arrows,yshift=0.1cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.1cm] {}
}
%classical vertical wire, absolute positioning
\newcommand{\vcwexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,xshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,xshift=-0.05cm] {}
}
%classical horizontal wire, absolute positioning
\newcommand{\vcwhexplicit}[2]{
	\arrow[from=#1,to=#2,arrows,yshift=0.05cm] {}\arrow[from=#1,to=#2,arrows,yshift=-0.05cm] {}
}
%quantum wire, absolute positioning, going to centres of cell, not edge.
\newcommand{\vqwexplicitcenter}[2]{
	\arrow[from=#1,to=#2,arrows,start anchor=center,end anchor=center] {}
}

%horizontal wires
\newcommand{\qw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows]{l}}{}}
\newcommand{\cw}{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{\arrow[arrows,yshift=0.05cm]{l}\arrow[arrows,yshift=-0.05cm]{l}}{}}
%define the strike distance for strike-through on qwbundle.
%\newcommand*{\StrikeDistance}{0.1cm}%
%a bundle of horizontal quantum wires
\newcommand{\qwbundle}[2][]{\ifthenelse{\the\pgfmatrixcurrentcolumn>1}{
	\def\helper{0}
	\pgfset{/quantikz,#1}
	\ifthenelse{\helper>0}{
		\arrow[arrows,yshift=0.1cm]{l}
		\ifthenelse{\helper=1}{\arrow[arrows]{l}}{}
		\arrow[arrows,yshift=-0.1cm]{l}
	}{
	\arrow[phantom,strike arrow]{l}[xshift=\pgfkeysvalueof{/quantikz/Strike Width}, yshift=\pgfkeysvalueof{/quantikz/Strike Height},anchor=south west,inner sep=0pt]{\scriptstyle #2}\qw
	}}{}}




%configure some of the style properties.
\tikzcdset{row sep/normal=0.5cm,column sep/normal=0.5cm,thick,nodes in empty cells,
	every cell/.style={
        anchor=center,minimum size=0pt,inner sep=0pt,outer sep=0pt,thick
    },
    arrows/.style={dash,thick},
    1-row diagram/.style={}
    }
\tikzset{
	thickness/.style={thick},
    operator/.style={draw,fill=white,minimum size=1.5em, inner sep=2pt,thickness,align=center},
    ggroup/.style={draw,minimum size=1.5em,thickness,align=center,inner sep=4pt},
    leftinternal/.style={anchor=mid west,font=\scriptsize,inner sep=4pt,align=center},
    rightinternal/.style={anchor=mid east,font=\scriptsize,inner sep=4pt,align=center},
    wave/.style={inner sep=-3pt,tape,fill=white,apply={draw=black} except on segments {5,6,1,2,9}},
    phase/.style={fill,shape=circle,minimum size=4pt},
    phase bundle/.style={fill,shape=rectangle,rounded corners=1.5pt,minimum width=4pt,minimum height=10pt},
    phase label/.style={label distance=2mm,anchor=mid,label position=45},
    ophase/.style={fill=white,draw=black,shape=circle,minimum size=4pt},
    internal/.style={thickness,black},
    line/.style={path picture={ 
\draw[internal](path picture bounding box.west) -- (path picture bounding box.east);
}},
	linecont/.style={circle,line},
    cross/.style={path picture={ 
\draw[internal](path picture bounding box.north) -- (path picture bounding box.south) (path picture bounding box.west) -- (path picture bounding box.east);
}},
    circlewc/.style={draw,circle,cross,minimum width=4pt,inner sep=3pt},
    crossx/.style={path picture={ 
\draw[internal,inner sep=0pt]
(path picture bounding box.south east) -- (path picture bounding box.north west) (path picture bounding box.south west) -- (path picture bounding box.north east) (path picture bounding box.west) -- (path picture bounding box.east);
}},
	crossx2/.style={circle,crossx,minimum size=1em},
	trash/.style={path picture={\draw[internal,inner sep=0pt,-stealth] (path picture bounding box.west) -- (path picture bounding box.center) -- (path picture bounding box.south);},minimum height=2.5em,minimum width=2em},
    dd/.style={decoration={brace},decorate,thickness},
    dm/.style={decoration={brace,mirror},decorate,thickness},
    slice/.style={thickness,red,dash pattern=on 5pt off 3pt,align=center},
    meter/.style={draw,fill=white,minimum width=2em,minimum height=1.5em, rectangle, font=\vphantom{A}, thickness,
 path picture={\draw ([shift={(.1,.24)}]path picture bounding box.south west) to[bend left=50] ([shift={(-.1,.24)}]path picture bounding box.south east);\draw[-{Latex[scale=0.6]}] ([shift={(0,.1)}]path picture bounding box.south) -- ([shift={(.3,-.1)}]path picture bounding box.north);}},
 	measuretab/.style={draw,signal,signal to=west,inner sep=4pt,fill=white},
 	meterD/.style={draw,rounded rectangle,rounded rectangle left arc=none,inner sep=4pt,fill=white},
 	measure/.style={draw,rounded rectangle,inner sep=4pt,fill=white},
 	my label/.style={yshift=0.1cm,above,align=center},
 	gg label/.style={label position=center,align=center},
 	group label/.style={label position=above,yshift=0.2cm,anchor=mid},
 	strike arrow/.style={
    decoration={markings, mark=at position 0.5 with {
        \draw [internal,-] 
            ++ (-\pgfkeysvalueof{/quantikz/Strike Width},-\pgfkeysvalueof{/quantikz/Strike Height} )
            -- ( \pgfkeysvalueof{/quantikz/Strike Width}, \pgfkeysvalueof{/quantikz/Strike Height});}	%can I use pgfkeys and do some maths here?
    },
    postaction={decorate},
}
}

\def\resetstyles{
\tikzcdset{thin,every cell/.append style={thin},arrows/.append style={thin}
    }
\tikzset{
	thickness/.style={thin},
	%operator/.append style={thin},
	%internal/.append style={thin},
	%dd/.append style={thin},
	%dm/.append style={thin},
	%slice/.append style={thin},
	meter/.append style={thin},
	phase/.append style={minimum size=3pt},
	ophase/.append style={minimum size=3pt},
	%circlewc/.append style={minimum size=3pt,inner sep=2pt}
}
}

\def\maketransparent{
\tikzset{
	operator/.append style={fill opacity=0},
	meter/.append style={fill opacity=0}
}
}
